Learning Influence Functions from Incomplete Observations

We study the problem of learning influence functions under incomplete observations of node activations. Incomplete observations are a major concern as most (online and real-world) social networks are not fully observable. We establish both proper and improper PAC learnability of influence functions under randomly missing observations. Proper PAC learnability under the Discrete-Time Linear Threshold (DLT) and Discrete-Time Independent Cascade (DIC) models is established by reducing incomplete observations to complete observations in a modified graph. Our improper PAC learnability result applies for the DLT and DIC models as well as the Continuous-Time Independent Cascade (CIC) model. It is based on a parametrization in terms of reachability features, and also gives rise to an efficient and practical heuristic. Experiments on synthetic and real-world datasets demonstrate the ability of our method to compensate even for a fairly large fraction of missing observations.

==> discussion-old.tex <==
So far, we have assumed that the \xhedit{retention rate} is the same for all the
nodes; however, our approach can be easily generalized to the case in
which each individual node has a different (but known) \xhedit{retention rate}.
The following theorem generalizes Theorems~\ref{Thm:DIC} and
\ref{Thm:DLT}. 
(The proofs of all theorems from this section are given in
Appendix~\ref{app:discussion-proofs}.)

\begin{theorem}\label{Thm:DiffLossRate}
Let $\lambda\in(0, 0.5)$ and for each node $v$, \xhedit{let $\RetRate_v$ be
$v$'s retention rate}. 
Write $\bar{r}=\frac{1}{n}\sum_{i=1}^n\frac{1}{\xhedit{\RetRate_v^2}}$.
\begin{itemize}
\item The class of influence functions under the DIC model 
in which all edge activation probabilities satisfy
$\EdgeW[e]\in [\lambda, 1-\lambda]$ is PAC learnable 
with sample complexity 
$\tilde{O}(\frac{\bar{r}^2\NodeNum^3 \EdgeNum}{\varepsilon^2})$.
\item The class of influence functions under the DLT model 
such that the edge weight for every edge satisfies
$\EdgeW[e]\in [\lambda, 1-\lambda]$,
and for every node $v$, 
$1 - \sum_{u\in N(v)}\EdgeWD{u}{v} \in [\lambda, 1-\lambda]$, 
is PAC learnable with sample complexity 
$\tilde{O}(\frac{\bar{r}^2\NodeNum^3 \EdgeNum}{\varepsilon^2})$. 
\end{itemize}
\end{theorem}
The empirical evaluation in the previous section also shows that the
performance does not change significantly if the true \xhedit{retention rate} of
each node is independently perturbed around the estimated mean \xhedit{retention rate}.

A second limitation of our approach is that we assume the \xhedit{retention rate 
\RetRate} to be known to the algorithm. 
Estimating \xhedit{\RetRate} in a real-world setting presents a ``chicken and
egg'' problem; however, we believe that a somewhat accurate estimate
of \xhedit{\RetRate} (perhaps based on past data for which ground truth can be
obtained at much higher cost) will still be a significant improvement
over the status quo, namely, pretending that no data are missing.  

Moreover, even approximate information about \xhedit{\RetRate} leads to
positive results on proper PAC learnability.
We show that the PAC learnability result can be extended to the case
where we only know that the true \xhedit{retention rate} lies in a given interval. 
\xhdelete{To simplify the notation, let $\RetRate = 1- \LossRate$ be the
retention rate, which is the probability that a node $v$'s activation is
observed.} Instead of knowing the exact value $\RetRate$, 
we only know that $\RetRate$ lies in an interval measured
by the relative error $\RelativeInterval$, namely \xhedit{$\RetRate\in I =
[\RetRateCenter\cdot(1-\RelativeInterval),
\RetRateCenter\cdot(1+\RelativeInterval)]$.}
Within that interval, the retention rate is adversarially
  chosen. We can then generalize Theorems~\ref{Thm:DIC} and
\ref{Thm:DLT} as follows.


\begin{theorem}\label{Thm:IntervalLossRate}
Let $\lambda\in(0, 0.5)$, and assume that the ground truth retention
rate $\RetRate$ is adversarially chosen in
\xhedit{$I = [\RetRateCenter\cdot(1-\RelativeInterval),
\RetRateCenter\cdot(1+\RelativeInterval)]$.}
For all $\varepsilon, \delta\in (0,1)$, 
all parametrizations of the diffusion model,  
and all distributions \SeedDist over seed sets \SeedSet: 
when given \emph{activation-only} and \emph{incomplete} training cascades
$\IncomCascs$, there exists a proper learning algorithm 
$\mathcal{A}$ which outputs an influence function $\InfFunc \in
\ModelClass$ satisfying:
$$
\Prob[\IncomCascs]{\Err[\InfFunc] - \Err[\InfFunc^*] \geq \varepsilon + \xhedit{\frac{4\RelativeInterval^2}{(1-\RelativeInterval)^2}}} \leq \delta.
$$
\begin{itemize}
\item For the DIC model, when all edge activation probabilities satisfy
$\EdgeW[e]\in [\lambda, 1-\lambda]$, 
the required number of observations is
\xhedit{$\CascNum=\max\{\tilde{O}(\frac{\NodeNum^3 \EdgeNum}{\varepsilon^2\RetRate^4}), \tilde{O}(\frac{\NodeNum^3 \EdgeNum \RelativeInterval^4}{\varepsilon^4\RetRate^4(1-\RelativeInterval)^4})\}$}.
\item For the DLT model, when all edges weights satisfy
$\EdgeW[e]\in [\lambda, 1-\lambda]$,
and for every node $v$, 
$1 - \sum_{u\in N(v)}\EdgeWD{u}{v} \in [\lambda, 1-\lambda]$, 
the required number of observations is
\xhedit{$\CascNum=\max\{\tilde{O}(\frac{\NodeNum^3 \EdgeNum}{\varepsilon^2\RetRate^4}), \tilde{O}(\frac{\NodeNum^3 \EdgeNum \RelativeInterval^4}{\varepsilon^4\RetRate^4(1-\RelativeInterval)^4})\}$}.
\end{itemize}
\end{theorem}

Notice that the result of Theorem~\ref{Thm:IntervalLossRate}
is not technically a PAC learnability result,
due to the additive error that depends on the interval
size.
However, the theorem provides useful approximation guarantees when the
interval size is small.
A dependence of the guarantee on the interval size is inevitable. 
For when nothing is known about the \xhedit{retention rate} (for $\RelativeInterval$
large enough), all information about the marginal activation
probabilities is lost in the incomplete data: 
for instance, if no nodes are ever obesrved active, we cannot
  distinguish the case $\RetRate = 0$ from the case in which no nodes
  become activated.
The experiments from the previous section confirm that for moderate
uncertainty about the \xhedit{retention rate}, the performance of our approach is
not very sensitive to the misestimation of \xhedit{\RetRate}.


==> experiment-old.tex <==
In this section, we experimentally evaluate the algorithm from
Section~\ref{Sec:algorithm}. Since no other methods explicitly
account for incomplete observations, we compare it to several
%  to incomplete observations in both
%synthetic and real-world cascade datasets. We compare our method to
%the following 
state-of-the-art methods for influence function learning with full
information.
%including both model-based two-step
%approaches~\cite{gomez-rodriguez_uncovering_2011,
%  praneeth_learning_2012} and the model-free influence function
%learner~\cite{du_influence_2014}. 
Hence, the main goal of the comparison is 
%\dkdelete{somehow unfair as
%the baseline methods are designed for complete cascades and we carry
%out the experiments}
to examine to what extent the impact of missing
data can be mitigated by being aware of it. 
We compare our algorithm to the following approaches:
%\begin{itemize}
%\item 
(1) \textbf{CIC} is an approach fitting the parameters of a CIC model,
%Two-step model-based approach where the delay parameters of the CIC
%model are inferred 
using the NetRate algorithm~\cite{gomez-rodriguez_uncovering_2011}
with exponential delay distribution.
%\item 
(2) \textbf{DIC} fits the activation probabilities of a DIC model
using the method in~\cite{praneeth_learning_2012}.
%\item 
(3) \textbf{InfluLearner} is the model-free approach proposed by Du et
al.~in \cite{du_influence_2014} and discussed in Section~\ref{Sec:algorithm}.
%without consideration of incomplete observation.
%\item 
(4) \textbf{Logistic} uses logistic regression to learn the influence functions 
$\InfFuncD{u}{\SeedSet}=f(\CharFuncV{\SeedSet}^{\top}\cdot\bm{c}_u + b)$
for each $u$ independently, 
where $\bm{c}_u$ is a learnable weight vector and 
$f(x)=\frac{1}{1+e^{-x}}$ is the logistic function.
%\item 
(5)\textbf{Linear} uses linear regression to learn the total influence
$\TotalInfFunc{\SeedSet}=\bm{c}^{\top}\cdot\CharFuncV{S}+ b$ of the set $S$.
Notice that the CIC and DIC methods have access to the 
\emph{activation time} of each node in addition to the final
activation status, giving them an inherent advantage.
%\end{itemize}

%When the total influence $\TotalInfFunc{\SeedSet}$ of a set of seeds $\SeedSet$ needs to be estimate, we apply an heuristic to add up the activation probabilities of all nodes that are not a seed for all methods except the linear regression, $\TotalInfFunc{\SeedSet} = |\SeedSet| + \sum_{v\in \NodeSet\backslash \SeedSet}\InfFuncD{v}{\SeedSet}$.
%\dkcomment{Why is this a heuristic? Isn't it exact? Do we need to say
%  this? Do we need to say this here?}

\subsection{Synthetic cascades}
\paragraph{Data generation.} We generate synthetic networks with
core-peripheral structure following the Kronecker graph
model~\cite{leskovec_kronecker_2010} with parameter matrix $[0.9, 0.5;
0.5, 0.3]$.\footnote{We also experimented on Kronecker graphs with
  hierarchical community structure ($[0.9, 0.1; 0.1, 0.9]$) and random
  structure ($[0.5, 0.5; 0.5 ,0.5]$). The results are similar and
  omitted due to space constraints.} 
Each generated network has $512$ nodes and $1024$ edges. 

We then generate synthetic cascades following the CIC, DIC and DLT models. 
For the CIC model, we use an exponential delay distribution on each
edge whose parameters are drawn independently and uniformly from $[0,1]$. 
The observation window length is $\ObvWin = 1.0$. 
For the DIC model, the activation probability for each edge is chosen
independently and uniformly from $[0, 0.4]$. 
For the DLT model, we follow~\cite{kempe_maximizing_2003} and set the
edge weight \EdgeWD{u}{v} as $1/d_v$ where $d_v$ is the in-degree of
node $v$. 
For each model, we generate $8192$ cascades as training data. 
The seed sets are sampled uniformly at random with sizes drawn from a
power law distribution with parameter $2.5$. 
The generated cascades have average sizes of $10.8$, $12.8$ and $13.0$ in
the CIC, DIC and DLT models, respectively. 
We then create incomplete cascades by varying the \xhedit{retention rate between $0.9$ and $0.1$}.  
The test set contains $200$ independently sampled seed sets generated
in the same way as the training data. 
To sidestep the computational cost of running Monte Carlo
simulations, we estimate the ground truth influence of the test seed sets
using the method proposed in~\cite{du_influence_2014}, with the true
model parameters. 
%\dkcomment{Are more details (commented out below) relevant here?}
%We set the number of graph samples to $500$ and number of label samples to $20$
%to guarantee the estimation achieve similar accuracy as running
%Monte-Carlo simulation.  

\paragraph{Algorithm settings.}
We apply all algorithms to cascades generated from all three
models; that is, we also consider the results under model misspecification.
Whenever applicable, we set the hyperparameters of the five comparison
algorithms to the ground truth values.
%For the model-based two-step approaches, we set the hyperparameters to
%the ground truth value as used in the cascades generation. This is, we
%set the observation window length to $1.0$ for the NetRate
%algorithm. However, 
When applying the NetRate algorithm to discrete-time cascades, 
we set the observation window to $10.0$. 
When applying the method in~\cite{praneeth_learning_2012} to
continuous-time cascades, we round activation times up to the nearest
multiple of 0.1, resulting in 10 discrete time steps.
%first split the observation window into
%ten intervals and the activation 
%time step is taken as the interval that the activation time lies
%in. 
For the model-free approaches (InfluLearner and our algorithm),
we use $\FeatureNum = 200$ features. 
%Moreover, it should be noticed that the
%two-step approaches naturally have an advantage over the model-free
%methods as they have access to not only the activated node set but
%also the exact time when a node was activated. 

\paragraph{Results.} 
Figure~\ref{Fig:syn_results} shows the Mean Absolute Error (MAE)
between the estimated total influence \TotalInfFunc{\SeedSet} and 
the true influence value, averaged over all testing seed sets.
For each setting (diffusion model and \xhedit{retention rate}), the reported MAE is
averaged over five independent runs. 
\begin{figure}
\begin{center}
\subfigure[CIC]{
\includegraphics[width=0.32\textwidth]{./figures/syn_CIC_ret.pdf}}
\subfigure[DIC]{
\includegraphics[width=0.32\textwidth]{./figures/syn_DIC_ret.pdf}}
\subfigure[DLT]{
\includegraphics[width=0.32\textwidth]{./figures/syn_DLT_ret.pdf}}
\end{center}
\caption{MAE of estimated influence as a function of the retention rate
  on synthetic datasets for (a) CIC model, (b) DIC model, (c) DLT model. 
  %under different level of incompleteness 
  %The $x$-axis is the loss rate and the $y$-axis the MAE. 
  The error bars shows one standard deviation.\label{Fig:syn_results}}
\end{figure}

The main insight is that accounting for missing observations indeed
strongly mitigates their effect: notice that \xhedit{down to retention rates} of
$0.5$, our algorithm can almost completely compensate for the data
loss, whereas both the model-free and parameter fitting approaches
deteriorate significantly even for \xhedit{large retention rates}.
For the parameter fitting approaches, even \xhedit{large retention rates} can lead to
missing and spurious edges in the inferred networks, and thus
significant estimation errors.
Additional observations include that fitting influence using (linear
or logistic) regression does not perform well at all, and that the CIC
inference approach appears more robust to model misspecification than
the DIC approach.

%From the results, we can clearly see the robustness of our approach
%compared to other methods under incomplete observations. Under all
%diffusion models, the accuracy of our method does not deteriorate much
%for a loss rate less than $0.5$. On the other hand, $20\%$ loss in the
%CIC and DIC models already have large impact for the model-based
%two-step approaches. As the model-based approach uses maximum
%likelihood estimation to infer the parameters of the diffusion
%process, the model misspecification due to the missing activation
%could lead to missing edges and also spurious edges in the diffusion
%networks, thus leading to large error in the estimated influence.  
%The model-based approach seems to be more robust under the DLT model. However, even under the DLT model, our method still significantly outperforms the baselines when loss rate is high. 
%%One possible explanation is that the model-based approaches are already under misspecification, and the impact of further incompleteness is smaller compared to that under the correct model. 

\paragraph{Sensitivity of retention rate.} 
We presented the algorithms as knowing \xhedit{\RetRate}.
Since \xhedit{\RetRate} itself is inferred from noisy data, it may be somewhat
misestimated.
Figure~\ref{Fig:uncertain} shows the impact of misestimating \xhedit{\RetRate}.
We generate synthetic cascades from all three diffusion models with a
true \xhedit{retention rate of $0.8$}, and then apply our algorithm with (incorrect) \xhedit{retention rate
$\RetRate \in \{1, 0.95, \ldots, 0.65, 0.6\}$}. 
The results are averaged over five independent runs. 
While the performance decreases as the misestimation gets worse
(after all, with \xhedit{$\RetRate = 1$}, the algorithm is basically the same as
InfluLearner), the degradation is graceful.
%method is not sensitive to the misspecification of loss rate. With
%$25\%$ error in estimating the loss rate, the MAE increases only by
%less than $10\%$. 
%\begin{figure}
%\begin{center}
%\includegraphics[width=0.5\textwidth]{./figures/uncertainty-crop.pdf}
%\end{center}
%\caption{Relative error in MAE under loss rate misspecification. X-axis shows the loss rate used in the algorithm. Y-axis is the relative different of MAW under misspecifided loss rate compared to that under true loss rate. \label{Fig:uncertain}}
%\end{figure}

\paragraph{Non-uniform retention rate}
In practice, different nodes may have different \xhedit{retention rates}, while we
are able only to estimate the mean \xhedit{retention rate \RetRate}.
For our experiments, we draw each node $v$'s \xhedit{retention rate
$\RetRate_v$} independently from a distribution with mean \xhedit{\RetRate}. 
Specifically, in our experiments, we use uniform and Gaussian
distributions;
for the uniform distribution, we draw
$\xhedit{\RetRate_v} \sim \text{Unif}[\xhedit{\RetRate}-\sigma, \xhedit{\RetRate}+\sigma]$;
for the Gaussian distribution, we draw
$\xhedit{\RetRate_v} \sim N(\xhedit{\RetRate}, \sigma^2)$, truncating draws at \xhedit{0 and 1}\footnote{\xhedit{The truncation could lead to bias on the mean of $\RetRate$. However empirical simulations show that the bias is only negligible, $0.01$ when $\sigma=0.2$.}}. 
In both cases, $\sigma$ measures the level of noise in the estimated
\xhedit{retention rate}. 
We set the mean \xhedit{retention rate $\RetRate$ to $0.8$} and vary
$\sigma$ in $\{0, 0.02, 0.05, 0.1, 0.2\}$. 
%We truncate the loss rate
%to interval $[0, 1]$ when $\LossRate_v$ is generated from the Gaussian
%distribution. 
Figure~\ref{Fig:random} shows the results for the Gaussian
distribution; the results of uniform distribution are similar 
and omitted. 
The results show that our model is very robust to random and
independent perturbations of individual \xhedit{retention rates} for each 
node.
\begin{figure}
\begin{center}
\includegraphics[width=0.5\textwidth]{./figures/random_Gaussian-crop.pdf}
\end{center}
\caption{Relative error in MAE when the true retention rates are drawn from
  the truncated Gaussian distribution. The $x$-axis shows standard deviation $\sigma$ of the retention
  rates from the mean, and the $y$-axis is the relative
  difference of the MAE compared to the case where all retention rates are
  the same and known. \label{Fig:random}}
\end{figure}


\subsection{Influence Estimation on real cascades}
We further evaluate the performance of our method on the real-world
MemeTracker\footnote{We use the preprocessed version of the
dataset released by Du et al.~\cite{du_influence_2014}
and available at
\url{http://www.cc.gatech.edu/~ndu8/InfluLearner.html}. \xhedit{Notice that the dataset is semi-real, as multi-node seed cascades are artificially created by merging single-node seed cascades.}} 
dataset \cite{leskovec2009meme}.
The dataset consists of the propagation of short textual phrases,
referred to as \emph{Memes}, via the publication of blog posts and
main-stream media news articles between March 2011 and February 2012.
Specifically, the dataset contains seven groups of cascades
corresponding to the propagation of Memes with certain keywords, 
namely ``apple and jobs'', ``tsunami earthquake'', ``william kate marriage''', 
``occupy wall-street'', ``airstrikes'', ``egypt'' and ``elections.''
Each cascade group consists of $1000$
nodes, with a number of cascades varying from $1000$ to $44000$.
We follow exactly the same evaluation method as
Du et al.~\cite{du_influence_2014} with a training/test set split of
60\%/40\%.

\begin{figure}[!t]
\minipage[t]{0.47\textwidth}
  \includegraphics[width=\linewidth]{./figures/uncertainty_ret-crop.pdf}
  \caption{Relative error in MAE under retention rate misspecification. 
    $x$-axis: retention rate \RetRate used by the algorithm. 
    $y$-axis: relative difference of MAE compared to using the true retention rate 0.8. 
   \label{Fig:uncertain}}
\endminipage\hfill
\minipage[t]{0.47\textwidth}
  \includegraphics[width=\linewidth]{./figures/real2-crop.pdf}
  \caption{MAE of influence estimation on seven sets of real-world cascades 
   with 20\% of activations missing. \label{Fig:real_results}}
\endminipage\hfill
\end{figure}


%\begin{figure}
%\begin{center}
%\includegraphics[width=0.5\textwidth]{./figures/real2-crop.pdf}
%\end{center}
%\caption{MAE of influence estimation on seven sets of real world cascades with $20\%$ activation missing. \label{Fig:real_results}}
%\end{figure}

To test the performance of influence function learning under
incomplete observations, we randomly delete 20\% of the
  occurrences, \xhedit{namely setting $\RetRate=0.8$}. 
%manually inject incompleteness into all
%the cascades with a loss rate of $20\%$. 
The results for other \xhedit{retention rates} are similar and omitted due to space constraints.
Figure~\ref{Fig:real_results} shows the MAE of our methods and the
five baselines, averaged over 100 random draws of test seed sets, for
all groups of memes.
While some baselines perform very poorly, even compared to the best
baseline (InfluLearner), our algorithm provides an 18\% reduction in
MAE (averaged over the seven groups), showing the potential of data
loss awareness to mitigate its effects.
%From the plot, we can clearly observe
%that the performance of our method is robust and consistently better
%than the baselines over all cascade groups. To be more specific, our
%method achieves a significant reduction of $18\%$ in MAE compared to
%the state-of-the-art method InfluLearner averaged over seven groups. 

